Improving students' code correctness and test completeness by informal specifications

The quality of software produced by students is often poor. How to teach students to develop good quality software has long been a topic in computer science education and research. We must conclude that we still do not have a good answer to this question. Specifications are necessary to determine the correctness of software, to develop error-free software and to write complete tests. Several attempts have been made to teach students to write specifications before writing code. So far, that has not proven to be very successful: Students do not like to write a specification and do not see the benefits of writing specifications. In this paper we focus on the use of informal specifications. Instead of teaching students how to write specifications, we teach them how to use informal specifications to develop correct software. The results were surprising: the number of errors in software and the completeness of tests both improved considerably and, most importantly, students really appreciate the specifications. We think that if students appreciate specification, we have a key to teach them how to specify and to appreciate its value.

==> futurework.tex <==
\section{Future work}\label{sec:future}
Of course, we have to find out whether our approach helps students to write specifications themselves in a later phase. 
We hope that they have learned, by the many examples of contracts, to see the gaps in the problem description.
They should be able to ask for more clarification when they are given a vague problem description or that they are able to draw up a complete contract in case of an incomplete contract.

We see two directions for further research. 
First, we wonder how we can better convince students of the added value of drawing up and using contracts. 
We will research this by offering more complex, real world assignments. For example, exercises: 
\begin{itemize}
	\item where one student draws up explicit specifications were another student codes the tests and/or implementation,
	\item with relative easy to read specifications, but ask for a complex algorithm to implement,
	\item in which a complex algorithm must be reviewed with and without accompanying specifications,
	\item in which parts of a project have to be refactored, with and without specifications. 
\end{itemize}
After students really understand the benefits of contracts, we can learn them how to draw specifications up. 

Second, in this study we see that the correctness of students' programs increases and that students appreciate the value of specifications. To what extent, however, students also have a better understanding of correctness after working with specifications is still unclear (\cite{kolikant2005students}). We will also research the misconception that take place, like the assumption that only one test cases is needed per subcontract \cite{Eldh-Analysis}.




